Revealing the Utilized Rank of Subspaces of Learning in Neural Networks

In this work, we study how well the learned weights of a neural network utilize the space available to them. This notion is related to capacity, but additionally incorporates the interaction of the network architecture with the dataset. Most learned weights appear to be full rank, and are therefore not amenable to low rank decomposition. This deceptively implies that the weights are utilizing the entire space available to them. We propose a simple data-driven transformation that projects the weights onto the subspace where the data and the weight interact. This preserves the functional mapping of the layer and reveals its low rank structure. In our findings, we conclude that most models utilize a fraction of the available space. For instance, for ViTB-16 and ViTL-16 trained on ImageNet, the mean layer utilization is 35% and 20% respectively. Our transformation results in reducing the parameters to 50% and 25% respectively, while resulting in less than 0.2% accuracy drop after fine-tuning. We also show that self-supervised pre-training drives this utilization up to 70%, justifying its suitability for downstream tasks.

==> 5Insights.tex <==

\section{Insights into Training Strategies From a Subspace Perspective}
\label{sec:insights}
In this section, we discuss some insights we gained from studying some popular training strategies and comment on potential explanations of their empirical success from a subspace perspective. 

% We believe that this formulation takes a step towards demystifying some of the empirically successful aspects of network architectures and hyperparameters, and we comment on a few in this section. %We only show graphs for a few layers of VGG11 trained on CIFAR10 here, with the rest shown in Appendix section \red{x}.

% \subsection{A closer look at the input subspace $S$, resulting in sparse weights. \red{TODO: improve title}}

% The subspace of the input at each layer warrants a deeper look. The first observation we make is that if the \textit{input}, $X \in \R^d$ lives in subspace $S$, we can modify the \textit{weight} in $S_\perp$ with the forward pass remaining largely unaltered, and therefore incurring little to no accuracy drop.

% To show this, let us alter the rows of W randomly in $S_\perp$. Let the dimension of $S$ be $k_S$, and the dimension $S_\perp$ be $k' = d-k_S$.
% Let $V_{S_\perp} \in \R^{k' \times d}$ contain the $k'$ bases of $S_\perp$ in its rows. If we pre-multiply $V_{S_\perp}$ by any random matrix of appropriate size, we remain in the row space of $V_{S_\perp}$, that is, we remain in $S_\perp$. Let us now alter W in $S_\perp$ using an appropriately sized random matrix, $A \in \mathbb{R}^{m \times (d-k_X)}$, such that the new weight $W' = W + AV_{S_\perp}$.  We now bound the error when replacing $W$ by $W'$:

% \begin{align}
% E &= XW^T  - X (W+A V_{S_\perp})^T \\
% &= XV_{S_\perp}^TA^T \\
% \|E\|^2 &\leq (1-e_S) \|X\|^2 \|A\|^2
% \end{align}


 
% This means that the error introduced can be driven down by choosing an appropriate energy/variance retention ratio for any such random matrix A. Note that this implies \textbf{that there infinitely many weights that do not change the neural network mapping that we can find analytically}, by moving the weight around randomly in $S_\perp.$ We show the effect of randomly varying W in $S_\perp$ for each layer in Figure \red{x}

    
    
%We are not going to talk about sparsity in this paper.
%SSSSSPARSITY:
% This can prove  useful in cases where the network size and the dataset complexity are mismatched, such as VGG19 trained in CIFAR10. (
% We know that VGG19 is too large, as evidenced by the fact that half of the layers can be removed without any drop in accuracy \red{(TBD: add IEEE ref)})
% In such cases, this observation prove quite useful since we can \textbf{craft an appropriate matrix A, analytically, that will result in structured sparsity in W}. We discuss one method of solving for this A to achieve sparsity in \red{Appendix section xx}, and show that we can zero out $k'$ out of $d$ columns in W that correspond to the independent columns of $V_{S_\perp}$. We can perform this calculation analytically, and hence do not need to retrain (or with limited finetuning). Additionally, this sparsity is structured and can be utilized without special purpose hardware changes. We discuss the resulting sparsity of some overparametrized nets in \red{section x} \red{mention SliceGPT comparison here}.







% \subsection{Looking at empirically successful strategies through a dimensional lens }
% We believe that this formulation takes a step towards demystifying some of the empirically successful aspects of network architectures and hyperparameters, and we comment on a few in this section. We only show graphs for a few layers of VGG11 trained on CIFAR10 here, with the rest shown in Appendix section \red{x}.


\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figures/wtdecay.jpeg}
    \vspace{-4mm}
    \caption{On the left, we show the histograms of the weights at initialization at end of learning for layer 7 of VGG11, CIFAR10 with and without weight decay. On the right, we show the spectral energy contribution of the same weights for layers 1 and 7 for different training epochs. }
    \label{fig:wt_decay}
\end{figure}


\subsection{The Role of Random Initialization} 
\label{insight:init}
Weights are initialized randomly with representation in both $S$ and $S_\perp$.
However, the gradients of $W$ are always in the span of the input, i.e. $S$.  This means that the gradient largely only updates $W$ and not $W_{S_\perp}$. In Figure \ref{fig:wt_decay}, we show the change in histograms of $W$, $W_S$ and $W_{S_\perp}$ from initialization to the end of training for the final layer of VGG11 trained on CIFAR10 with a utilized rank of $62/512$.

%While we find $S$ and $S_\perp$ at the end of training, we want to see how the contribution of $W$ to each space changes between initialization and end of training by looking at the change in histograms of $W, W_s$ and $W_{s_\perp}$. 
For the case without weight decay, we note see that while the distributions for $W$ and $W_S$ change distribution, $W_{s_\perp}$ remains largely unchanged since it does not get any gradient updates. This is the `un-utilized' part of $W$ that arises as a consequence of random initialization. We can also observe this in Figure \ref{fig:wt_decay}, where we plot the spectral energy contribution (indicated by norm ratios) of $W_S$ and $W_{S_\perp}$.
 % This ratio captures the spectral energy contribution of weight in $S$ and $S_\perp$. 
At epoch 0, the network is randomly initialized and the contribution of $W_S$ and $W_{S_\perp}$ is directly the ratio of their dimensions, shown by the green and red dots. However, as we perform gradient descent, the weight only updates in $S$ and therefore the contribution of $W_S$ grows and far outweighs the contribution $W_{S_\perp}$ at the end of training.  Since $X$ largely exists in $X_S$, the forward pass interaction between $X$ and $W_{S_\perp}$ is negligible. \textbf{Hence, the weights initialized in $S_\perp$ don't contribute to learning significantly, and don't get updated}.  This implies that there are low rank initializations that would converge to the same accuracy if we a priori knew the subspace $S$ at initialization, potentially forming a subspace of lottery tickets \cite{lth, lowranklth}. % \
%\red{ToDo: show you can project on S, and alter Sperp at init and learn to same accuracy}

% \begin{figure}[t]
%    \begin{floatrow}
%     \ffigbox{\includegraphics[width=0.5\textwidth]{Figures/vert_WD0hist7.png}}
%      {\caption{Histograms of W, $W_s$ and $W_{s_\perp}$ at the beginning and end of training.
%      }
%      \label{fig:vert_hist} }
%           \ffigbox{\includegraphics[width=0.45\textwidth]{Figures/wt_decay.png}}
%      {\caption{Norms of $W_s$ and $W_{s_\perp}$ relative to W through training, with and without weight decay}\label{fig:wt_decay} }
% \end{floatrow}
% \end{figure}



% We show the histogram of weights in S and $S_\perp$ at random initialization and after training in Figure \red{xx}. It is easy to see that the weights in S grow during training, but the weight in $S_\perp$ remain the same. As a fun experiment, inspired by the question asked for coordinate networks in \red{simon Lucey init paper}, \red{expt TBD: we introduce a hidden smiley/cipher/song in a network and train it, and show that he smiley/cipher/song remains unaltered.} We believe this answers the question posed in the paper. This can also be used as a low effort method to hide a trademark in $S_\perp$, however, any attacker with knowledge of the network and dataset can still steal the network and erase it. Lastly, we also believe that there is a link between this formulation and lottery tickets that we will explore for future work. 
 %ref[Fig 3 of https://proceedings.mlr.press/v202/ramasinghe23a/ramasinghe23a.pdf] 


\subsection{Weight Decay drives $\mathbf{W_{S_\perp}}$ towards zero}
Recent works \cite{wd1, wd2} show that the traditional understanding of weight decay as regularization does not explain its impact. Previously, we showed that since the gradient lives in the subspace of the input $S$, any weight initialized in $S_\perp$ does not get any gradient. While that is true for losses such as cross-entropy, regularization losses such as weight decay do provide a gradient to $W_{S_\perp}$, driving it towards zero. Since $W_{S_\perp}$ does not have a competing gradient from the target loss, the weight in $S_\perp$ is able to get smaller and smaller, thus indeed biasing the network to a smaller rank overall. We can see this from Figure \ref{fig:wt_decay}, as the difference in the histograms for $W_{S_\perp}$ between weight decay on and off. When the weight decay is off, the histogram of $W_{S_\perp}$ does not change between initialization and at the end of training, but the variance gets smaller when weight decay is on.  We also note this in Figure \ref{fig:wt_decay}. When weight decay is turned off (dotted line), $S_\perp$ contributes a significantly higher proportion of energy at the end of training without weight decay (0.45 vs 0.2 with weight decay for layer 7), resulting in a larger selected dimension of $S$. The corresponding MLU goes from 47\% to 64\% when weight decay is turned off. \textbf{Thus weight decay does indeed seem to bias the network towards low rank representations by way of diminishing the weights in $\mathbf{S_\perp}$}. The connection between weight-decay and low-rank bias is also supported by experiments studying neural rank collapse \cite{rankcollapse}.



\subsection{Non-Linearity redistributes spectral energy}
For full utilization of the weight-space available, we want the column space of $W$ to overlap fully with the input subspace. Therefore, the larger the dimension of $S$, the more the learning potential at that layer. We know that stacked linear layers in an MLP without non-linearity cannot expand dimensions due to the sub-multiplicative nature of rank. Hence, it falls to the non-linearity to expand the dimensions from the output of the previous layer to the input of the next layer. However, the most popular non-linearity, ReLU, is an orthant projection that cannot ostensibly expand dimensions. To understand this, we plot the spectral energy pre- and post-ReLU for different layers of VGG11 trained on CIFAR10. We find that \textbf{the destruction of information from zeroing out data not in the positive orthant allows ReLU to redistribute spectral energy in more dimensions, thus facilitating learning in larger dimensions in the next layers}.
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figures/relu.png}
    \vspace{-4mm}
    \caption{The spectral energy spread of the first 4 layers of a trained VGG11 on CIFAR10 pre and post ReLU. The dotted lines separate S and $S_\perp$ for 99\% spectral energy.}
    \label{fig:enter-label}
    \vspace{-2mm}
\end{figure}
% Since the gradient for the columns of W is also in the same subspace S, larger dimensional S implies a larger utilization of the capacity available at W.% Most other commonly used non-linearites are variants of ReLU that mimic it's behavior. We show that SiLU used in ViTs, for instance, performs similar redistribution as can be seen from Appendix section \red{x}.

\subsection{Skip Connections expand learnable dimensions and mixup spans them densely}
\paragraph{Skip Connections} Suppose the input to a layer lives in a subspace of rank $k_S$ and the weight lives in  a different subspace of rank $k_W$ such that $k_W < k_S$. This would imply that a lot of the spectral energy of X does not get utilized at that layer. However, skip connections allow X to be part of the input to a later layer, allowing for its unused dimensions to be used at the later layer. At the later layer, the input subspace $S$ is consequently larger because it is the addition of two distinct subspaces, and thus the network has the potential to learn in a larger subspace than in feedforward networks. From Table \ref{tab:cf10}, we note that ResNet-style architectures have consistently higher MLU than VGG style networks, even at $10\times$ the depth. 
\vspace{-1mm}
\paragraph{Input and Activation Mixup} Our analysis implies that to be effective on a validation dataset, we need to use training data that lives in the same subspace, since the gradients will also limit themselves to this subspace. This is relevant for data augmentation strategies. Mixup \cite{mixup}, at both the input and activation level uses a linear combination of inputs, which remains in the same subspace, and hence the gradient that results from the augmented data effects the subspace in which the real data lives. Hence, it does not expand dimensions, but helps span it more densely. 


% \subsection{What the intrinsic rank of W captures: \red{Do we want to go here? Maybe not. Leave this for paper which studies the dynamics of space overlap during training}}
% We now attempt to explain why the intrinsic rank of the weight matrix is lower than the actual rank. 

% The input $X \in \mathbb{R}^{B \times d}$, lives in a subspace S of rank $k_X$. Let's consider $W \in \mathbb{R}^{m \times d}$. W has m rows in $ \mathbb{R}^{d}$, and W is full rank at initialization. Let us assume that the true rank of W, perhaps coming from the fact that $m \leq d$ is $k_W$, and the row space of W is R. We have the interaction of input in subspace S of d-dimensional space, and W in subspace T of d-dimensional spaces. These spaces might or might not be perfectly overlapping, and let's say the rank of intersection of S and R is $k_SR$. The forward pass can then be written as 

% \begin{align}
% \label{eq:expanded_RS}
% Y&=(X_S + X_{S_\perp}) (W_R + W_{R_\perp} )^T \\
% &= X_S W_R^T + X_{S_\perp} W_R^T  + X_S W_{R_\perp}^T + X_{S_\perp} W_{R_\perp}^T \\
% &= X_{SR} W_{SR}^T + X_{\overline{S}R} W_{\overline{S}R}^T  + X_{S\overline{R}} W_{S\overline{R}}^T + X_{\overline{S}\overline{R}} W_{\overline{S}\overline{R}}^T \\
% Y &= Y_{SR} + Y_{\overline{S}R} + Y_{S\overline{R}} + Y_{\overline{S}\overline{R}} \\
% \|Y\|^2 &= \|Y_{SR}\|^2 + \|Y_{\overline{S}R}\|^2 + \|Y_{S\overline{R}}\|^2 + Y_{\overline{S}\overline{R}}\|^2
% \end{align}

% The last step follows from the fact that the 4 spaces partition the whole of $\mathbb{R}^d$ without intersecting with each other. Refer to venn diagram xx.
% It is easy to see that most of the energy of Y lies in SR. Let us bound the error of $ Y - Y_SR$
% %TODO: ensure these are all squares  of norms

% \begin{align}
% E  &= Y - Y_{SR} \\
% &= Y_{\overline{S}R} + Y_{S\overline{R}} + Y_{\overline{S}\overline{R}} \\ 
% \| E \|^2 &=  \|Y_{\overline{S}R}\|^2 + \|Y_{S\overline{R}} \|^2+ Y_{\overline{S}\overline{R}}\|^2 \\
% \|Y_{\overline{S}R}\|^2 &\leq \|X_{\overline{S}R}\|^2 \|W_{\overline{S}R}\|^2  
% \leq  \|X_{\overline{S}}\|^2\|W_{R}\|^2  
% \leq  0.01\|X\|^2\|W\|^2 ;\\
% \|Y_{S\overline{R}}\|^2 &\leq \|X_{S\overline{R}}\|^2 \|W_{S\overline{R}}\|^2  
% \leq  \|X_S\|^2\|W_{\overline{R}}\|^2  
% \leq  0.01\|X\|^2\|W\|^2 ;\\
% \|Y_{\overline{S}\overline{R}}\|^2 &\leq \|X_{\overline{S}\overline{R}}\|^2 \|W_{\overline{S}\overline{R}}\|^2 
% \leq  \|X_{\overline{S}} \|^2 \|W_{\overline{R}}\|^2  = 0.0001\|X\|^2\|W\|^2 \\
% \implies \|E \|^2 &\leq 0.0201 \|X\|^2\|W\|^2
% \end{align}



% This means that the space of intersection of S and R (of the input and the weights respectively) dictates the intrinsic rank. Further, within this space of intersection, we are only interested in the subspace that captures most of the energy of interaction between W and X, and that sis captured by the SVD of the output Y. The rank of Y captures the concentration of energy of the space where W and X meaningfully interact. 



% \subsection{Dynamics of the Learning Subspaces - not in this paper no}
% We now study how the intrinsic rank develops during the course of learning. We study this for VGG19 for CIFAR10 since it contains both over and underparametrized layers (as evidenced by the ability to remove the last 6 layers without any change in accuracy upon retraining/finetuning).


==> Tables/CF10_RN50_scalewidth.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{ResNet50 statistics on CIFAR10 when scaling base width (\#filters) in each layer.}
\label{tab:rn50_cf10_width}
% \addtolength{\tabcolsep}{-0.3pt}
\def\arraystretch{1.3}%
\begin{tabular}{|c|ccccc|}
\hline
\rowcolor[HTML]{B0B3B2} 
Base Width                 & Accuracy (\%) & ALU (\%) & Total Prms(M) & Utilized Prms(M) & Prms Ratio \\ \hline
\cellcolor[HTML]{D4D4D4}8  & 81.0          & 86       & 0.4            & 0.4                 & 0.98         \\
\cellcolor[HTML]{D4D4D4}16 & 86.2          & 78       & 1.5            & 1.1                 & 0.74         \\
\cellcolor[HTML]{D4D4D4}32 & 87.0          & 58       & 5.9            & 2.2                 & 0.37         \\
\cellcolor[HTML]{D4D4D4}48 & 86.3          & 50       & 13.3           & 4.0                 & 0.30         \\
\cellcolor[HTML]{D4D4D4}64 & 86.7          & 43       & 23.6           & 5.5                 & 0.23         \\ \hline
\end{tabular}
\end{table}

==> Tables/CF10_RN50_scalewidth_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{ResNet50 statistics on CIFAR10 when scaling base width (\#filters) in each layer.}
\label{tab:rn50_cf10_width_old}
\begin{tabular}{|cccccc|}
\hline
\rowcolor[HTML]{B0B3B2} 
\begin{tabular}[c]{@{}c@{}}Base\\ Width\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total\\ Prms(M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Utilized\\ Prms(M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Utilized\\ Prms \%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Average \\ Layer Util\end{tabular} & Accuracy \\ \hline
\cellcolor[HTML]{D4D4D4}8                            & 0.38                                                    & 0.37                                                       & 98\%                                                       & 86\%                                                          & 81.0     \\
\cellcolor[HTML]{D4D4D4}16                           & 1.50                                                    & 1.11                                                       & 74\%                                                       & 78\%                                                          & 86.2     \\
\cellcolor[HTML]{D4D4D4}32                           & 5.93                                                    & 2.21                                                       & 37\%                                                       & 58\%                                                          & 87.0     \\
\cellcolor[HTML]{D4D4D4}48                           & 13.29                                                   & 4.03                                                       & 30\%                                                       & 50\%                                                          & 86.3     \\
\cellcolor[HTML]{D4D4D4}64                           & 23.58                                                   & 5.53                                                       & 23\%                                                       & 43\%                                                          & 86.7     \\ \hline
\end{tabular}
\end{table}

==> Tables/CF_results_color.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\caption{Results for Intrinsic Rank Decomposition on CIFAR dataset for different architectures. FT refers to finetuning and Savings refer to ratio of original to decomposed parameters \red{finetuning tbd,anticipate less than 1 percent acc drop for everything}}
\label{tab:cf10}
\addtolength{\tabcolsep}{1pt}
\def\arraystretch{1.15}%
\begin{tabular}{|c|c|cc|cc|cc|}
\hline
 &
  Architecture &
  \begin{tabular}[c]{@{}c@{}}Orig Acc\\  (\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Orig ALU\\  (\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc - Ours\\ (\%) ($\Delta$)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}True ALU\\  (\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Params\\  Ratio\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}FLOPs\\ Ratio\end{tabular} \\ \hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{CIFAR10}}  & VGG11            & 91.5 & 98 & 92.5 (+1.0) & 47 & 0.34 & 0.60 \\
                          & VGG13            & 92.9 & 98 & 93.5 (+0.6) & 47 & 0.24 & 0.60 \\
                          & VGG16            & 93.2 & 99 & 93.6 (+0.4) & 44 & 0.18 & 0.54 \\
                          & VGG19            & 92.7 & 99 & 93.6 (+0.9) & 32 & 0.11 & 0.38 \\
                          & ResNet18         & 90.9 & 95 & 91.4 (+0.5) & 80 & 0.86 & 0.92 \\
                          & ResNet50         & 92.8 & 96 & 93.1 (+0.3) & 64 & 0.78 & 0.78 \\
                          & ResNet101        & 93.2 & 96 & 94.1 (+0.9) & 51 & 0.73 & 0.64 \\ \hline
\multirow{9}{*}{\rotatebox[origin=c]{90}{CIFAR100}} & VGG11            & 66.9 & 99 & 67.4 (+0.5) & 64 & 0.78 & 0.72 \\
                          & VGG13            & 70.2 & 99 & 71 (+0.8)   & 68 & 0.76 & 0.77 \\
                          & VGG16            & 70.2 & 99 & 71.4 (+1.2) & 62 & 0.61 & 0.71 \\
                          & VGG19            & 70.2 & 99 & 71.8 (+1.6) & 51 & 0.38 & 0.68 \\
                          & ResNet18         & 66.0 & 96 & 67.8 (+1.8) & 90 & 0.98 & 0.99 \\
                          & ResNet50         & 71.4 & 96 & 73.5 (+2.1) & 80 & 0.93 & 0.92 \\
                          & ResNet101        & 72.2 & 96 & 73.5 (+1.3) & 63 & 0.87 & 0.77 \\
                          & WideResNet50\_2  & 81.2 & 99 & 80.6 (-0.6) & 43 & 0.68 & 0.58 \\
                          & WideResNet101\_2 & 82.3 & 99 & 81.7 (-0.6) & 33 & 0.51 & 0.44 \\ \hline
\end{tabular}
\end{table}

==> Tables/CF_results_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Results for Intrinsic Rank Decomposition on CIFAR dataset for different architectures. FT refers to finetuning and Savings refer to ratio of original to decomposed parameters \red{finetuning tbd,anticipate less than 1 percent acc drop for everything}}
\label{tab:cf10}
\addtolength{\tabcolsep}{-0.8pt}
\def\arraystretch{1.15}%
\begin{tabular}{|
>{\columncolor[HTML]{D4D4D4}}c |
>{\columncolor[HTML]{D4D4D4}}c ccccccc|}
\hline
\cellcolor[HTML]{B0B3B2}                           & \cellcolor[HTML]{B0B3B2}Network & \cellcolor[HTML]{B0B3B2}Orig Acc & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank \\Acc (no FT)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank \\Acc (FT)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}Acc\\Drop\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}Orig\\Prms(M)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank \\ Prms (M)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}Savings \end{tabular} \\ \hline
\cellcolor[HTML]{D4D4D4}                           & vgg11                       & 91.3                           & 90.9                                                                                          &                                                                                            & 0.4                            & 9.2                                                                                & 3.6                                                                                   & 2.6                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg13                       & 92.9                           & 92.3                                                                                          &                                                                                            & 0.6                            & 9.4                                                                                & 2.7                                                                                   & 3.5                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg16                       & 93.1                           & 92.4                                                                                          &                                                                                            & 0.7                            & 14.7                                                                               & 3.1                                                                                   & 4.7                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg19                       & 92.6                           & 91.7                                                                                          &                                                                                            & 0.8                            & 20.1                                                                               & 2.9                                                                                   & 7.0                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & resnet18                   & 89.9                           & 88.9                                                                                          &                                                                                            & 1.0                            & 11.2                                                                               & 5.2                                                                                   & 2.2                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & resnet50                   & 89.5                           & 87.1                                                                                          &                                                                                            & 2.4                            & 23.6                                                                               & 5.5                                                                                   & 4.3                                                                                                \\
\multirow{-7}{*}{\cellcolor[HTML]{D4D4D4}\rotatebox[origin=c]{90}{CIFAR10}}  & resnet101                  & 89.8                           & 85.0                                                                                          &                                                                                            & 4.8                            & 42.6                                                                               & 11.7                                                                                  & 3.6                                                                                                \\ \hline
\cellcolor[HTML]{D4D4D4}                           & vgg11                       & 66.8                           & 66.5                                                                                          &                                                                                            & 0.3                            & 9.3                                                                                & 9.4                                                                                   & 1.0                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg13                       & 70.1                           & 70.0                                                                                          &                                                                                            & 0.1                            & 9.5                                                                                & 8.0                                                                                   & 1.2                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg16                       & 70.0                           & 69.4                                                                                          &                                                                                            & 0.7                            & 14.8                                                                               & 11.8                                                                                  & 1.3                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & vgg19                       & 70.0                           & 69.4                                                                                          &                                                                                            & 0.6                            & 20.1                                                                               & 7.6                                                                                   & 2.6                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & resnet18                   & 67.9                           & 67.4                                                                                          &                                                                                            & 0.5                            & 11.2                                                                               & 8.4                                                                                   & 1.3                                                                                                \\
\cellcolor[HTML]{D4D4D4}                           & resnet50                   & 66.2                           & 64.1                                                                                          &                                                                                            & 2.1                            & 23.8                                                                               & 14.3                                                                                  & 1.7                                                                                                \\
\multirow{-7}{*}{\cellcolor[HTML]{D4D4D4}\rotatebox[origin=c]{90}{CIFAR100}} & resnet101                  & 67.7                           & 62.6                                                                                          &                                                                                            & 5.0                            & 42.8                                                                               & 26.4                                                                                  & 1.6                                                                                                \\ \hline
\end{tabular}
\end{table}

==> Tables/CF_results_wtihcolor.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Results for Intrinsic Rank Decomposition on CIFAR dataset for different architectures. FT refers to finetuning }
\label{tab:cf10}
\addtolength{\tabcolsep}{1.3pt}
\def\arraystretch{1.2}%
\begin{tabular}{@{}|c|c|cc|cc|cc|@{}}
\toprule
Dataset &
  Architecture &
  \begin{tabular}[c]{@{}c@{}}Orig Acc\\  (\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc - Ours\\ (\%) ($\Delta$)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}True ALU\\  (\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Params\\  Ratio\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}FLOPs\\ Ratio\end{tabular} \\ \midrule
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG11            & 91.5 & 98 & 92.5 (+1.0) & 47 & 0.34 & 0.60 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG13            & 92.9 & 98 & 93.5 (+0.6) & 47 & 0.24 & 0.60 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG16            & 93.2 & 99 & 93.6 (+0.4) & 44 & 0.18 & 0.54 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG19            & 92.7 & 99 & 93.6 (+0.9) & 32 & 0.11 & 0.38 \\ \cmidrule(l){2-8} 
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}ResNet18         & 90.9 & 95 & 91.4 (+0.5) & 80 & 0.86 & 0.92 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}ResNet50         & 92.8 & 96 & 93.1 (+0.3) & 64 & 0.78 & 0.78 \\
\multirow{-7}{*}{\cellcolor[HTML]{D4D4D4}\rotatebox[origin=c]{90}{CIFAR10}}  & \cellcolor[HTML]{D4D4D4}ResNet101        & 93.2 & 96 & 94.1 (+0.9) & 51 & 0.73 & 0.64 \\ \midrule
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG11            & 66.9 & 99 & 67.4 (+0.5) & 64 & 0.78 & 0.72 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG13            & 70.2 & 99 & 71 (+0.8)   & 68 & 0.76 & 0.77 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG16            & 70.2 & 99 & 71.4 (+1.2) & 62 & 0.61 & 0.71 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}VGG19            & 70.2 & 99 & 71.8 (+1.6) & 51 & 0.38 & 0.68 \\ \cmidrule(l){2-8} 
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}ResNet18         & 66.0 & 96 & 67.8 (+1.8) & 90 & 0.98 & 0.99 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}ResNet50         & 71.4 & 96 & 73.5 (+2.1) & 80 & 0.93 & 0.92 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}ResNet101        & 72.2 & 96 & 73.5 (+1.3) & 63 & 0.87 & 0.77 \\
\cellcolor[HTML]{D4D4D4}                           & \cellcolor[HTML]{D4D4D4}WideResNet50\_2  & 81.2 & 99 & 80.6 (-0.6) & 43 & 0.68 & 0.58 \\
\multirow{-9}{*}{\cellcolor[HTML]{D4D4D4}\rotatebox[origin=c]{90}{CIFAR100}} & \cellcolor[HTML]{D4D4D4}WideResNet101\_2 & 82.3 & 99 & 81.7 (-0.6) & 33 & 0.51 & 0.44 \\ \cmidrule(l){2-8} 
\end{tabular}
\end{table}

==> Tables/ImNet_results_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer pResNetation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Results for Intrinsic Rank Decomposition on ImageNet dataset for different architectures. FT refers to finetuning and Savings refer to ratio of original to decomposed parameters \red{finetuning tbd,anticipate less than 1 percent acc drop for everything, and the savings will increase if we only decompose when advantageous. Stil have to decompose attention layers, savings will go up after that.}}
\label{tab:imnet}
\addtolength{\tabcolsep}{-1pt}
\def\arraystretch{1.15}%
\begin{tabular}{|
>{\columncolor[HTML]{D4D4D4}}c ccccccc|}
\hline
\cellcolor[HTML]{B0B3B2}Network & \cellcolor[HTML]{B0B3B2}Orig  Acc & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank \\ Acc (no FT)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank \\ Acc (FT)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}Acc\\ Drop\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}Orig\\ Prms(M)\end{tabular} & \cellcolor[HTML]{B0B3B2}\begin{tabular}[c]{@{}c@{}}LowRank\\ Prms(M)\end{tabular} & \cellcolor[HTML]{B0B3B2}Savings \\ \hline
ViTB16                      & 81.1                              & 78.9                                                                                   &                                                                                     & 2.1                                                                        & 86.6                                                                           & 72.9                                                                              & 1.2                             \\
ViTB32                      & 75.9                              & 73.9                                                                                   &                                                                                     & 2.0                                                                        & 88.2                                                                           & 72.4                                                                              & 1.2                             \\
ViTL16                      & 79.7                              & 76.4                                                                                   &                                                                                     & 3.2                                                                        & 304.3                                                                          & 174.7                                                                             & 1.7                             \\
ViTL32                      & 77.0                              & 73.0                                                                                   &                                                                                     & 4.0                                                                        & 306.5                                                                          & 209.9                                                                             & 1.5                             \\
ViTB16(FT-Lin)             & 81.9                              & 80.0                                                                                   &                                                                                     & 1.9                                                                        & 86.6                                                                           & 101.4                                                                             & 0.9                             \\
ViTB16(FT-e2e)             & 85.3                              & 81.3                                                                                   &                                                                                     & 4.0                                                                        & 86.9                                                                           & 315.0                                                                             & 0.3                             \\
ViTL16(FT-Lin)             & 85.1                              & 83.5                                                                                   &                                                                                     & 1.7                                                                        & 304.3                                                                          & 93.4                                                                              & 3.3                             \\
ViTL16(FT-e2e)             & 88.1                              & 84.0                                                                                   &                                                                                     & 4.0                                                                        & 305.2                                                                          & 283.2                                                                             & 1.1                             \\
ResNet18                        & 69.8                              & 68.3                                                                                   &                                                                                     & 1.5                                                                        & 11.7                                                                           & 11.1                                                                              & 1.1                             \\
ResNet34                        & 73.3                              & 70.6                                                                                   &                                                                                     & 2.7                                                                        & 21.8                                                                           & 19.3                                                                              & 1.1                             \\
ResNet50                        & 80.9                              & 76.7                                                                                   &                                                                                     & 4.1                                                                        & 25.6                                                                           & 23.5                                                                              & 1.1                             \\
ResNet101                       & 81.9                              & 73.9                                                                                   &                                                                                     & 8.0                                                                        & 44.5                                                                           & 34.3                                                                              & 1.3                             \\
ResNet152                       & 82.3                              & 70.8                                                                                   &                                                                                     & 11.5                                                                       & 60.2                                                                           & 40.2                                                                              & 1.5                             \\
Wide ResNet101              & 82.5                              & 74.1                                                                                   &                                                                                     & 8.4                                                                        & 126.9                                                                          & 69.7                                                                              & 1.8                             \\
Wide ResNet50               & 81.6                              & 76.9                                                                                   &                                                                                     & 4.7                                                                        & 68.9                                                                           & 53.9                                                                              & 1.3                             \\ \hline
\end{tabular}
\end{table}
